Software Pipelining for Quantum Loop Programs

We propose a method for performing software pipelining on quantum for-loop programs, exploiting parallelism in and across iterations. We redefine concepts that are useful in program optimization, including array aliasing, instruction dependency and resource conflict, this time in optimization of quantum programs. Using the redefined concepts, we present a software pipelining algorithm exploiting instruction-level parallelism in quantum loop programs. The optimization method is then evaluated on some test cases, including popular applications like QAOA, and compared with several baseline results. The evaluation results show that our approach outperforms loop optimizers exploiting only in-loop optimization chances by reducing total depth of the loop program to close to the optimal program depth obtained by full loop unrolling, while generating much smaller code in size. This is the first step towards optimization of a quantum program with such loop control flow as far as we know.

==> qasm/xyqcirc.tex <==
%
% File:   xyqcirc.tex
% Date:   14-Mar-04
% Author: I. Chuang <ichuang@mit.edu>
%
% Definitions for producing quantum circuits with XYPIC in latex
%
% $Log: xyqcirc.tex,v $
% Revision 1.17  2004/03/25 05:01:23  ike
% discard and slash
%
% Revision 1.16  2004/03/25 04:58:42  ike
% added discard, and variable width dmeter
%
% Revision 1.15  2004/03/24 23:43:33  ike
% \dmeter and \sq
%
% Revision 1.14  2004/03/24 20:29:40  ike
% added \t for swap
%
% Revision 1.13  2004/03/24 17:52:16  ike
% removed \w from \gspace
%
% Revision 1.12  2004/03/24 16:38:34  ike
% added small space before |0> for \z
%
% Revision 1.11  2004/03/24 16:23:11  ike
% added \z
%
% Revision 1.10  2004/03/24 16:19:11  ike
% added multiple qubit operations
%
% Revision 1.9  2004/03/24 03:03:44  ike
% typo
%
% Revision 1.8  2004/03/24 02:50:09  ike
% added qv
%
% Revision 1.7  2004/03/24 00:07:34  ike
% add \m matrix op
%
% Revision 1.6  2004/03/23 23:13:10  ike
% misc
%
% Revision 1.5  2004/03/23 23:12:42  ike
% works now
%
% Revision 1.4  2004/03/23 22:22:34  ike
% ifthen also failes - because xymatrix entries in \save...\restore
%
% Revision 1.3  2004/03/23 21:34:36  ike
% no q/c wire switching
%
% Revision 1.2  2004/03/23 21:25:29  ike
% classical qo quantum wire switching try
%
% Revision 1.1  2004/03/23 21:01:46  ike
% Initial revision
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preliminaries

\usepackage{graphicx}

\usepackage[frame,line,arrow,matrix,tips]{xy}	% all that is usually necessary
\usepackage{tikz}
\usetikzlibrary{fit, backgrounds, matrix, arrows.meta}
\newcommand{\emptybullet}{
\begin{tikzpicture}
\filldraw[fill=white,draw=black] circle (3pt);
\end{tikzpicture}
}
\CompilePrefix{xygui-}
\makeindex
\pagestyle{empty}

\setlength{\oddsidemargin}{-0.5in}	% 1.25in left margin 
\setlength{\evensidemargin}{-0.5in}	% 1.25in left margin (even pages)

\setlength{\topmargin}{0.0in}		% 1in top margin
\setlength{\textwidth}{6.25in}		% 6.0in text - 1.25in rt margin
\setlength{\textheight}{8.6in}		% Body ht for 1in margins
\addtolength{\topmargin}{-\headheight}	% No header, so compensate
\addtolength{\topmargin}{-\headsep}	% for header height and separation

\begin{document}

\thispagestyle{empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% wires

\def\w{\ar@{-}[l]}
\def\W{\ar@{=}[l]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% labels

% simple label
\def\A#1{\save []="#1" \restore}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% single qubit operations

\def\op#1{*+[F]{\rule[-0.2ex]{0ex}{2.1ex}#1}}	% operator in box
\def\b{*={\bullet}}
\def\wb{*+<1.5pt,1.5pt>{\emptybullet}}
\def\o{*={\oplus}}
\def\t{*={\times}}				% for swap gate
\def\sq{*=<6pt,6pt>[F]{}}			% square, for controlled-phase
\def\m#1{\left[\matrix{#1}\right]}		% matrix shortcut
\def\z{*+[]{\rule[-0.2ex]{0ex}{2.1ex}~|0\>}}	% re-init to |0>
\def\discard{*[]{\rule[-0.2ex]{0.75pt}{2.1ex}~}}	% vertical ``|''
\def\slash{*={/}}				% slash for wire bundles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% nop's

\def\N{*-{}\W}
\def\n{*-{}\w}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% misc definitions

\def\>{\rangle}
\def\<{\langle}
\def\ua{\uparrow}

% measurement box
\def\meter{*+[]{\put(-3,0){\includegraphics[scale=.5]{meter.epsf}}~~~~}%
		\ar@{-}[l]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% qubit names (and also revert to qubit wires, vs, cbit wires)

\def\q#1{*+{\rule[-0.2ex]{0ex}{2.1ex}|#1\>}}
\def\qv#1#2{*+{\rule[-0.2ex]{0ex}{2.1ex}|#1\>=|#2\>}}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% multiple qubit gates

% utulity text box for figuring out width of things
\newbox{\sbox}

% empty space of width determined by the text argument
\def\gspace#1{*+{\rule[-0.2ex]{0ex}{2.1ex}%
	\setbox\sbox=\hbox{$#1$}%
	\hspace*{\wd\sbox}}}
	
% n-qubit operation #1=box label, #2=number of qubits (eg d=2 qubits, ddd=4)
\def\gnqubit#1#2{\gspace{#1}
		 \save [].[#2]!C="qq"*[F]\frm{}\restore
		 \save "qq"*[]{#1} \restore}

% two-qubit operation
\def\gtwo#1{\gnqubit{#1}{d}}

% two-qubit operation
\def\gthree#1{\gnqubit{#1}{dd}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ``D'' style measurement gate a-la-cleve, at Michael Nielsen's request

\def\dmeterwide#1#2{*{\xy <0pt,-8pt>;<0pt,8pt> **@{-};
		    <0pt,-8pt>;<#2,-8pt> **@{-} ;
		    <0pt, 8pt>;<#2, 8pt> **@{-} ;
		    <#2,0pt>-<5pt,0pt>*{#1} ;
		    <#2,0pt>*\cir<8pt>{r_l}\endxy}}

\def\dmeter#1{\dmeterwide{#1}{12pt}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

